The effect of stock market indexing on corporate tax avoidance

Membership in the Russell 1000 and 2000 Indices is based on a ranking of market capitalization in May. Each index is separately value weighted such that firms just inside the Russell 2000 are comparable in size to firms just outside (i.e. at the bottom of the Russell 1000) but have much higher index weights. These features allow for the the annual reconstitution of these indices to be used as part of a regression discontinuity design to identify the effect of stock market indexing. Using this design, I investigate whether stock market indexing affects corporate tax avoidance. I find no evidence that firms just inside the Russell 2000 have significantly different effective tax rates than firms just outside.

==> iortax2.tex <==
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{$\text{R2000}_{i,t}$}&\multicolumn{1}{c}{$\text{R2000}_{i,t}$}&\multicolumn{1}{c}{$\text{CETR}_{i,t}$}&\multicolumn{1}{c}{$\text{CETR}_{i,t}$}&\multicolumn{1}{c}{$\text{GETR}_{i,t}$}&\multicolumn{1}{c}{$\text{GETR}_{i,t}$}\\
\hline
$\tau_{i,t}$        &       0.870\sym{***}&       0.861\sym{***}&                     &                     &                     &                     \\
                    &     (0.021)         &     (0.023)         &                     &                     &                     &                     \\
$\tau_{i,t}\times\text{May Rank (Add)}_{i,t}$&       0.000         &                     &                     &                     &                     &                     \\
                    &     (0.000)         &                     &                     &                     &                     &                     \\
$\text{May Rank (Add)}_{i,t}$&       0.000\sym{***}&                     &       0.000         &                     &      -0.000         &                     \\
                    &     (0.000)         &                     &     (0.000)         &                     &     (0.000)         &                     \\
$\tau_{i,t}\times\text{May Rank (Del)}_{i,t}$&                     &      -0.000\sym{**} &                     &                     &                     &                     \\
                    &                     &     (0.000)         &                     &                     &                     &                     \\
$\text{May Rank (Del)}_{i,t}$&                     &       0.001\sym{***}&                     &       0.000         &                     &      -0.000         \\
                    &                     &     (0.000)         &                     &     (0.000)         &                     &     (0.000)         \\
$\text{R2000}_{i,t}$&                     &                     &      -0.024         &      -0.020         &       0.031         &      -0.004         \\
                    &                     &                     &     (0.025)         &     (0.017)         &     (0.021)         &     (0.015)         \\
$\text{May Rank (Add)}_{i,t}\times\text{R2000}_{i,t}$&                     &                     &      -0.000         &                     &       0.000         &                     \\
                    &                     &                     &     (0.000)         &                     &     (0.000)         &                     \\
$\text{May Rank (Del)}_{i,t}\times\text{R2000}_{i,t}$&                     &                     &                     &      -0.000         &                     &       0.000         \\
                    &                     &                     &                     &     (0.000)         &                     &     (0.000)         \\
Constant            &       0.056\sym{***}&       0.083\sym{***}&       0.264\sym{***}&       0.212\sym{***}&       0.279\sym{***}&       0.288\sym{***}\\
                    &     (0.012)         &     (0.020)         &     (0.015)         &     (0.012)         &     (0.011)         &     (0.011)         \\
\hline
Observations        &        2255         &        3027         &        1817         &        2635         &        1817         &        2635         \\

